Design and performance of the silicon sensors for the CMS barrel pixel detector

The CMS experiment at the LHC includes a hybrid silicon pixel detector for the reconstruction of charged tracks and of the interaction vertices. The barrel region consists of n-in-n sensors with 100X150 um^2 cell size processed on diffusion oxygenated float zone silicon. A biasing grid is implemented and pixel isolation is achieved with the moderated p-spray technique. An extensive test program was carried out on the H2 beam line of the CERN SPS. In this paper we describe the sensor layout, the beam test setup and the results obtained with both irradiated and non-irradiated prototype devices. Measurements of charge collection, hit detection efficiency, Lorentz angle and spatial resolution are presented.

==> electrical_measurements.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Electrical measurements\label{sec:electrical}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
